Learning to Re-weight Examples with Optimal Transport for Imbalanced Classification

Imbalanced data pose challenges for deep learning based classification models. One of the most widely-used approaches for tackling imbalanced data is re-weighting, where training samples are associated with different weights in the loss function. Most of existing re-weighting approaches treat the example weights as the learnable parameter and optimize the weights on the meta set, entailing expensive bilevel optimization. In this paper, we propose a novel re-weighting method based on optimal transport (OT) from a distributional point of view. Specifically, we view the training set as an imbalanced distribution over its samples, which is transported by OT to a balanced distribution obtained from the meta set. The weights of the training samples are the probability mass of the imbalanced distribution and learned by minimizing the OT distance between the two distributions. Compared with existing methods, our proposed one disengages the dependence of the weight learning on the concerned classifier at each iteration. Experiments on image, text and point cloud datasets demonstrate that our proposed re-weighting method has excellent performance, achieving state-of-the-art results in many cases and providing a promising tool for addressing the imbalanced classification issue.

==> 2022 imbalance OT/backup_table.tex <==
%备份一些表格数据

%sst2
\begin{table}[!ht]
\centering
\vspace{3mm}
\caption{{Comparison of the proposed model and {baselines} trained with different proportions on SST-2, where the number of examples in the validation set is 10 for each class. $*$ indicates results reported in original paper. $\dag$ indicates results reported in \cite{liu2021improving}}.}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccc}% {p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
\toprule[1pt]
\textbf{Method} & 100 : 1000 & 50 : 1000 & 20 : 1000 & 10 : 1000 \\ \hline
\textbf{BERT Baseline (Without Fine Tuned)}&  74.91$\pm$4.62&53.26$\pm$5.70&50.54$\pm$1.40& 49.84$\pm$0.02\\
\textbf{BERT Baseline (Fine Tuned)}&  81.64$\pm$3.79& 75.53$\pm$1.90&65.23$\pm$3.91&60.61$\pm$5.00\\
\textbf{Baseline}&  78.25$\pm$2.24& 57.18$\pm$1.88&55.00$\pm$1.23&50.17$\pm$1.34\\
\textbf{Proportion  $\dag$} & 79.59$\pm$3.35&\XSolidBrush&78.76$\pm$2.40 &60.63$\pm$13.13\\
\textbf{Hu et al.'s $*$ \cite{hu2019learning}} &81.57$\pm$0.74 &79.35$\pm$2.59 &73.61$\pm$11.86 &	55.84$\pm$11.84 \\
\textbf{Hu et al.'s+Regularization $*$ \cite{hu2019learning}} &82.25$\pm$1.16 &\XSolidBrush&79.53$\pm$1.64 &	66.68$\pm$13.99 \\
\textbf{Liu et al.'s $*$\cite{liu2021improving}}& 82.58$\pm$0.98 &\XSolidBrush& 81.14$\pm$1.25& 80.62$\pm$0.93\\
\textbf{Logit Adjustment $\tau=1.0$ \cite{menon2020long}}& 79.23$\pm$1.68&71.19$\pm$2.09&56.16$\pm$15.45&49.50$\pm$17.11\\
\textbf{LDAM-DRW \cite{}}&78.89$\pm$4.89&66.30$\pm$13.92&65.17$\pm$10.88&53.89$\pm$17.70\\
% \textbf{Only Stage 1}& 78.258 & 75.057 & 55.032 & 49.655 \\
% \textbf{Stage 1 + Stage 2}& 75.891 & 68.056 & 51.989 & 49.655\\
\textbf{Our model+self-attention (score)+OT loss(label)}& 86.48$\pm$0.29&86.30$\pm$0.37 & 86.19$\pm$0.54 &86.03$\pm$0.46 \\
\textbf{Our model+self-attention (score)+OT loss(feature)}&86.08$\pm$3.80 &86.08$\pm$3.71 &85.98$\pm$2.85  &85.95$\pm$4.72 \\
\textbf{Our model+self-attention (score)+OT loss(label+feature)}& 86.71$\pm$0.24 & 86.49$\pm$0.60 & 86.47$\pm$0.51 &86.24$\pm$0.60\\

\textbf{Our model+self-attention (score)+OT loss(label+feature) + val + Dynamic Balance}& \textbf{87.08$\pm$0.09} & \textbf{87.13$\pm$0.04} & \textbf{87.14$\pm$0.08} & \textbf{87.10$\pm$0.05}\\

\textbf{Our model+self-attention (score)+OT loss(label+feature) + noval + Dynamic Balance}& \textbf{87.12$\pm$0.03} & \textbf{87.11$\pm$0.01} & \textbf{87.09$\pm$0.07} & \textbf{87.12$\pm$0.01}\\

\textbf{Our model+self-attention (score)+OT loss(label)+OT loss(feature)}& 86.59$\pm$0.50 & 86.14$\pm$0.52 & 86.08$\pm$0.77 & 85.85$\pm$0.52\\
\bottomrule
\end{tabular}}\label{sst2}
\end{table}

%sst5
\begin{table}[!ht]
\centering
\vspace{3mm}
\caption{{Comparison of the proposed model and {baselines} trained with different proportions on SST-5 for multi-classification, where the number of examples in the validation set is 10 for each class. Overall, there are 500 samples for the majority classes.}}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccc}% {p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
\toprule[1pt]
\textbf{Method} & 75 : 500 & 60 : 500 & 50 : 500\\ \hline
\textbf{BERT Baseline (Fined Tuned)}& 43.76$\pm$0.77&43.25$\pm$0.73&42.70$\pm$0.52 \\
\textbf{Baseline}& 36.99$\pm$0.46&36.75$\pm$0.43&36.46$\pm$0.50\\
\textbf{Proportion} & \XSolidBrush  & \XSolidBrush & 42.59$\pm$1.12\\
\textbf{19NIPS Hu et al.’s} &\XSolidBrush  & \XSolidBrush & 39.82$\pm$1.07\\
\textbf{19NIPS Hu et al.’s+R} &\XSolidBrush  &\XSolidBrush  & 40.14$\pm$0.39\\
\textbf{22ICLR} & \XSolidBrush  & \XSolidBrush  & 44.62$\pm$1.08\\
\textbf{Our model+self-attention (score)+OT loss(label)+OT loss(feature)}&44.95$\pm$0.56&44.79$\pm$0.82&44.68$\pm$1.16\\
\textbf{Our model+self-attention (score)+OT loss(label + feature)}&44.95$\pm$0.56&44.79$\pm$0.82&44.68$\pm$1.16\\
\bottomrule
\end{tabular}}\label{sst5}
\end{table}






% \begin{table}
% \caption{\small{Test top-1 errors(\%) of ResNet-50 on ImageNet-LT.  $*$ indicates results reported in original paper.}}\label{placeslt}
% \centering
% \begin{tabular}{c|c}
% \toprule[1pt]
% \textbf{Method} & \textbf{ALL}\\ \hline
% \textbf{Cross Entropy (CE)}& 61.12\\
% \textbf{Class Balanced CE } \cite{cui2019class} (results from \cite{liu2019large})&59.15 \\
% \textbf{$\text{OLTR}$ \cite{liu2019large}}&59.64\\
% \textbf{$\text{LDAM}$ }&58.14\\
% LDAM-DRW & 54.26 \\
% \textbf{$\text{Mets-class-weight with CE loss}$\cite{jamal2020rethinking}}&55.08\\
% MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% % \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% % \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
% \textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.50}\\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}
\caption{\small{Test top-1 errors(\%) on ImageNet-LT using  ResNet-50. $*$ indicates results from  \cite{li2021metasaug}.}}\label{imagenet}
\centering
\begin{tabular}{c|cc}
\toprule[1pt]
\textbf{Method} & \textbf{ImageNet-LT}\\ \hline
{Cross Entropy (CE)}& 61.12\\
$\text{Class Balanced CE}^*$\cite{cui2019class}&59.15 \\
$\text{OLTR}^*$\cite{liu2019large} &59.64\\
{$\text{LDAM}^*$ \cite{cao2019learning}}&58.14\\
{$\text{LDAM}^*$ \cite{cao2019learning}} & 54.26 \\
{$\text{Mets-class-weight with CE loss}^*$\cite{jamal2020rethinking}}&55.08\\
MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.40}\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{\small{Test top-1 errors(\%) on ImageNet-LT using  ResNet-50. $*$ indicates results from  \cite{li2021metasaug}.}}\label{imagenet}
\centering
\begin{tabular}{c|cc}
\toprule[1pt]
\textbf{Method} & \textbf{ImageNet-LT}\\ \hline
{Cross Entropy (CE)}& 61.12\\
$\text{Class Balanced CE}^*$\cite{cui2019class}&59.15 \\
$\text{OLTR}^*$\cite{liu2019large} &59.64\\
{$\text{LDAM}^*$ \cite{cao2019learning}}&58.14\\
{$\text{LDAM}^*$ \cite{cao2019learning}} & 54.26 \\
{$\text{Mets-class-weight with CE loss}^*$\cite{jamal2020rethinking}}&55.08\\
MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.40}\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{\small{Test top-1 errors(\%) of ResNet-152 on Places-LT. \textbf{ALL} indicates that we evaluate and compare methods on the whole training dataset. $*$ indicates results reported in original paper.}}\label{placeslt}
\centering
\begin{tabular}{c|c}
\toprule[1pt]
\textbf{Method} & \textbf{ALL}\\ \hline
Cross Entropy (CE)& 69.3\\
$\text{Mets-class-weight with CE loss}$$*$\cite{jamal2020rethinking}&69.2\\
Focal loss \cite{lin2017focal} (results from \cite{liu2019large})& 65.4 \\
$\text{OLTR}$$*$ \cite{liu2019large}&64.1\\
$\text{cRT}$$*$ \cite{DBLP:conf/iclr/KangXRYGFK20} & 63.3\\
$\text{MetaSAug with LDAM loss}$ \cite{li2021metasaug} & \\
$\text{LWS}$$*$ \cite{DBLP:conf/iclr/KangXRYGFK20} & 62.4\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{60.6}\\
\bottomrule
\end{tabular}
\end{table}

==> backup_table.tex <==
%备份一些表格数据

%sst2
\begin{table}[!ht]
\centering
\vspace{3mm}
\caption{{Comparison of the proposed model and {baselines} trained with different proportions on SST-2, where the number of examples in the validation set is 10 for each class. $*$ indicates results reported in original paper. $\dag$ indicates results reported in \cite{liu2021improving}}.}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccc}% {p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
\toprule[1pt]
\textbf{Method} & 100 : 1000 & 50 : 1000 & 20 : 1000 & 10 : 1000 \\ \hline
\textbf{BERT Baseline (Without Fine Tuned)}&  74.91$\pm$4.62&53.26$\pm$5.70&50.54$\pm$1.40& 49.84$\pm$0.02\\
\textbf{BERT Baseline (Fine Tuned)}&  81.64$\pm$3.79& 75.53$\pm$1.90&65.23$\pm$3.91&60.61$\pm$5.00\\
\textbf{Baseline}&  78.25$\pm$2.24& 57.18$\pm$1.88&55.00$\pm$1.23&50.17$\pm$1.34\\
\textbf{Proportion  $\dag$} & 79.59$\pm$3.35&\XSolidBrush&78.76$\pm$2.40 &60.63$\pm$13.13\\
\textbf{Hu et al.'s $*$ \cite{hu2019learning}} &81.57$\pm$0.74 &79.35$\pm$2.59 &73.61$\pm$11.86 &	55.84$\pm$11.84 \\
\textbf{Hu et al.'s+Regularization $*$ \cite{hu2019learning}} &82.25$\pm$1.16 &\XSolidBrush&79.53$\pm$1.64 &	66.68$\pm$13.99 \\
\textbf{Liu et al.'s $*$\cite{liu2021improving}}& 82.58$\pm$0.98 &\XSolidBrush& 81.14$\pm$1.25& 80.62$\pm$0.93\\
\textbf{Logit Adjustment $\tau=1.0$ \cite{menon2020long}}& 79.23$\pm$1.68&71.19$\pm$2.09&56.16$\pm$15.45&49.50$\pm$17.11\\
\textbf{LDAM-DRW \cite{}}&78.89$\pm$4.89&66.30$\pm$13.92&65.17$\pm$10.88&53.89$\pm$17.70\\
% \textbf{Only Stage 1}& 78.258 & 75.057 & 55.032 & 49.655 \\
% \textbf{Stage 1 + Stage 2}& 75.891 & 68.056 & 51.989 & 49.655\\
\textbf{Our model+self-attention (score)+OT loss(label)}& 86.48$\pm$0.29&86.30$\pm$0.37 & 86.19$\pm$0.54 &86.03$\pm$0.46 \\
\textbf{Our model+self-attention (score)+OT loss(feature)}&86.08$\pm$3.80 &86.08$\pm$3.71 &85.98$\pm$2.85  &85.95$\pm$4.72 \\
\textbf{Our model+self-attention (score)+OT loss(label+feature)}& 86.71$\pm$0.24 & 86.49$\pm$0.60 & 86.47$\pm$0.51 &86.24$\pm$0.60\\

\textbf{Our model+self-attention (score)+OT loss(label+feature) + val + Dynamic Balance}& \textbf{87.08$\pm$0.09} & \textbf{87.13$\pm$0.04} & \textbf{87.14$\pm$0.08} & \textbf{87.10$\pm$0.05}\\

\textbf{Our model+self-attention (score)+OT loss(label+feature) + noval + Dynamic Balance}& \textbf{87.12$\pm$0.03} & \textbf{87.11$\pm$0.01} & \textbf{87.09$\pm$0.07} & \textbf{87.12$\pm$0.01}\\

\textbf{Our model+self-attention (score)+OT loss(label)+OT loss(feature)}& 86.59$\pm$0.50 & 86.14$\pm$0.52 & 86.08$\pm$0.77 & 85.85$\pm$0.52\\
\bottomrule
\end{tabular}}\label{sst2}
\end{table}

%sst5
\begin{table}[!ht]
\centering
\vspace{3mm}
\caption{{Comparison of the proposed model and {baselines} trained with different proportions on SST-5 for multi-classification, where the number of examples in the validation set is 10 for each class. Overall, there are 500 samples for the majority classes.}}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|cccccc}% {p{0.1cm}p{0.1cm}p{0.1cm}p{0.1cm}}
\toprule[1pt]
\textbf{Method} & 75 : 500 & 60 : 500 & 50 : 500\\ \hline
\textbf{BERT Baseline (Fined Tuned)}& 43.76$\pm$0.77&43.25$\pm$0.73&42.70$\pm$0.52 \\
\textbf{Baseline}& 36.99$\pm$0.46&36.75$\pm$0.43&36.46$\pm$0.50\\
\textbf{Proportion} & \XSolidBrush  & \XSolidBrush & 42.59$\pm$1.12\\
\textbf{19NIPS Hu et al.’s} &\XSolidBrush  & \XSolidBrush & 39.82$\pm$1.07\\
\textbf{19NIPS Hu et al.’s+R} &\XSolidBrush  &\XSolidBrush  & 40.14$\pm$0.39\\
\textbf{22ICLR} & \XSolidBrush  & \XSolidBrush  & 44.62$\pm$1.08\\
\textbf{Our model+self-attention (score)+OT loss(label)+OT loss(feature)}&44.95$\pm$0.56&44.79$\pm$0.82&44.68$\pm$1.16\\
\textbf{Our model+self-attention (score)+OT loss(label + feature)}&44.95$\pm$0.56&44.79$\pm$0.82&44.68$\pm$1.16\\
\bottomrule
\end{tabular}}\label{sst5}
\end{table}






% \begin{table}
% \caption{\small{Test top-1 errors(\%) of ResNet-50 on ImageNet-LT.  $*$ indicates results reported in original paper.}}\label{placeslt}
% \centering
% \begin{tabular}{c|c}
% \toprule[1pt]
% \textbf{Method} & \textbf{ALL}\\ \hline
% \textbf{Cross Entropy (CE)}& 61.12\\
% \textbf{Class Balanced CE } \cite{cui2019class} (results from \cite{liu2019large})&59.15 \\
% \textbf{$\text{OLTR}$ \cite{liu2019large}}&59.64\\
% \textbf{$\text{LDAM}$ }&58.14\\
% LDAM-DRW & 54.26 \\
% \textbf{$\text{Mets-class-weight with CE loss}$\cite{jamal2020rethinking}}&55.08\\
% MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% % \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% % \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
% \textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.50}\\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}
\caption{\small{Test top-1 errors(\%) on ImageNet-LT using  ResNet-50. $*$ indicates results from  \cite{li2021metasaug}.}}\label{imagenet}
\centering
\begin{tabular}{c|cc}
\toprule[1pt]
\textbf{Method} & \textbf{ImageNet-LT}\\ \hline
{Cross Entropy (CE)}& 61.12\\
$\text{Class Balanced CE}^*$\cite{cui2019class}&59.15 \\
$\text{OLTR}^*$\cite{liu2019large} &59.64\\
{$\text{LDAM}^*$ \cite{cao2019learning}}&58.14\\
{$\text{LDAM}^*$ \cite{cao2019learning}} & 54.26 \\
{$\text{Mets-class-weight with CE loss}^*$\cite{jamal2020rethinking}}&55.08\\
MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.40}\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}
\caption{\small{Test top-1 errors(\%) on ImageNet-LT using  ResNet-50. $*$ indicates results from  \cite{li2021metasaug}.}}\label{imagenet}
\centering
\begin{tabular}{c|cc}
\toprule[1pt]
\textbf{Method} & \textbf{ImageNet-LT}\\ \hline
{Cross Entropy (CE)}& 61.12\\
$\text{Class Balanced CE}^*$\cite{cui2019class}&59.15 \\
$\text{OLTR}^*$\cite{liu2019large} &59.64\\
{$\text{LDAM}^*$ \cite{cao2019learning}}&58.14\\
{$\text{LDAM}^*$ \cite{cao2019learning}} & 54.26 \\
{$\text{Mets-class-weight with CE loss}^*$\cite{jamal2020rethinking}}&55.08\\
MetaSAug with CE loss \cite{li2021metasaug}&52.61\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{52.40}\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\caption{\small{Test top-1 errors(\%) of ResNet-152 on Places-LT. \textbf{ALL} indicates that we evaluate and compare methods on the whole training dataset. $*$ indicates results reported in original paper.}}\label{placeslt}
\centering
\begin{tabular}{c|c}
\toprule[1pt]
\textbf{Method} & \textbf{ALL}\\ \hline
Cross Entropy (CE)& 69.3\\
$\text{Mets-class-weight with CE loss}$$*$\cite{jamal2020rethinking}&69.2\\
Focal loss \cite{lin2017focal} (results from \cite{liu2019large})& 65.4 \\
$\text{OLTR}$$*$ \cite{liu2019large}&64.1\\
$\text{cRT}$$*$ \cite{DBLP:conf/iclr/KangXRYGFK20} & 63.3\\
$\text{MetaSAug with LDAM loss}$ \cite{li2021metasaug} & \\
$\text{LWS}$$*$ \cite{DBLP:conf/iclr/KangXRYGFK20} & 62.4\\
% \textbf{$\text{DisAlign}$\cite{zhang2021distribution}}&60.7\\
% \textbf{Our model+self-attention (score)+OT loss(label + feature)}&\\
\textbf{Our model+ w/o-attention+OT loss(label + feature)}&\textbf{60.6}\\
\bottomrule
\end{tabular}
\end{table}
